Dijet production in $\sqrt{s}=7$ TeV $pp$ collisions with large rapidity gaps at the ATLAS experiment

A $6.8 \ {\rm nb^{-1}}$ sample of $pp$ collision data collected under low-luminosity conditions at $\sqrt{s} = 7$ TeV by the ATLAS detector at the Large Hadron Collider is used to study diffractive dijet production. Events containing at least two jets with $p_\mathrm{T} > 20$ GeV are selected and analysed in terms of variables which discriminate between diffractive and non-diffractive processes. Cross sections are measured differentially in $\Delta\eta^F$, the size of the observable forward region of pseudorapidity which is devoid of hadronic activity, and in an estimator, $\tilde{\xi}$, of the fractional momentum loss of the proton assuming single diffractive dissociation ($pp \rightarrow pX$). Model comparisons indicate a dominant non-diffractive contribution up to moderately large $\Delta\eta^F$ and small $\tilde{\xi}$, with a diffractive contribution which is significant at the highest $\Delta\eta^F$ and the lowest $\tilde{\xi}$. The rapidity-gap survival probability is estimated from comparisons of the data in this latter region with predictions based on diffractive parton distribution functions.

==> ddijets-metadata.tex <==
%-------------------------------------------------------------------------------
% This file contains the title, author and abstract.
% It also contains all relevant document numbers used by the different cover pages.
%-------------------------------------------------------------------------------

% Title
\newcommand{\ddijetstitle}{{Dijet production in {\boldmath $\sqrt{s}=7$} \TeV\ 
{\boldmath $pp$} collisions with large rapidity gaps at the ATLAS experiment}}
\AtlasTitle{\ddijetstitle}

% Author - this does not work with revtex (add it after \begin{document})
\author{The ATLAS Collaboration}

% Date: if not given, uses current date
%\date{\today}

% ATLAS reference code, to help ATLAS members to locate the paper
\AtlasRefCode{STDM-2014-04}

% ATLAS note number. Can be an COM, INT, PUB or CONF note
 \AtlasNote{ATL-COM-PHYS-2015-202}
% \AtlasNote{ATL-PHYS-PUB-2014-XXX}
% \AtlasNote{ATL-COM-PHYS-2014-XXX}

% CERN preprint number
\PreprintIdNumber{CERN-PH-EP-2015-227}

% ATLAS date - arXiv submission; to be filled in by the Physics Office
\AtlasDate{\today}

% arXiv identifier
% \arXivId{14XX.YYYY}

% HepData record
% \HepDataRecord{ZZZZZZZZ}

% Submission journal and final reference
 \AtlasJournal{PLB}
% \AtlasJournalRef{\PLB 789 (2014) 123}
% \AtlasDOI{}

\AtlasAbstract{%
A $6.8 \ {\mathrm nb^{-1}}$ sample of $pp$ collision data collected under 
low-luminosity conditions
at $\sqrt{s} = 7$ \TeV\ by the ATLAS detector at the Large Hadron Collider is 
used to study diffractive dijet production. Events containing at least two jets 
with $p_\mathrm{T} > 20$ \GeV\ are selected and analysed in terms of 
variables which discriminate between diffractive and non-diffractive processes.
Cross sections are measured differentially in $\detaf$, the size of the 
observable forward region of pseudorapidity which is devoid of hadronic 
activity, and in an estimator, $\xiepz$, of the fractional momentum loss
of the proton assuming single diffractive dissociation ($pp \rightarrow pX$). 
Model comparisons indicate a
dominant non-diffractive contribution up to moderately large 
$\detaf$ and small $\xiepz$, with a diffractive contribution which 
is significant at the highest $\detaf$ and the lowest $\xiepz$. The 
rapidity-gap survival probability is estimated from comparisons of the data in 
this latter region with predictions based on diffractive parton distribution 
functions.}

%-------------------------------------------------------------------------------
% The following information is needed for the cover page. The commands are only defined
% if you use the coverpage option in atlasdoc or use the atlascover package
%-------------------------------------------------------------------------------

% List of supporting notes  (leave as null \AtlasCoverSupportingNote{} if you want to skip this option)
%\AtlasCoverSupportingNote{}
%\AtlasCoverSupportingNote{ATL-COM-PHYS-2014-1363}{https://cds.cern.ch/record/1956329}
%\AtlasCoverSupportingNote{Short title note 2}{https://cds.cern.ch/record/YYYYYYY}
%
% OR (the 2nd option is deprecated, especially for CONF and PUB notes)
%
% Supporting material TWiki page  (leave as null \AtlasCoverTwikiURL{} if you want to skip this option)
% \AtlasCoverTwikiURL{https://twiki.cern.ch/twiki/bin/view/Atlas/WebHome}

% Comment deadline
\AtlasCoverCommentsDeadline{12 October 2015}

% Analysis team members - contact editors should no longer be specified
% as there is a generic email list name for the editors
\AtlasCoverAnalysisTeam{Hardeep Bansil, Oldrich Kepka, Vlastimil Kus, Paul 
Newman, Marek Tasevsky}

% Editorial Board Members - indicate the Chair by a (chair) after his/her name
% Give either all members at once (then they appear on one line), or separately
\AtlasCoverEdBoardMember{Lauren Tompkins~(chair), Christopher Meyer, Christophe
Royon, Andrew Hamiltion}
% \AtlasCoverEdBoardMember{EdBoard~Chair~(chair)}
% \AtlasCoverEdBoardMember{EB~Member~1}
% \AtlasCoverEdBoardMember{EB~Member~2}
% \AtlasCoverEdBoardMember{EB~Member~3}

% A PUB note has readers and not an EdBoard -- give their names here (one line or several entries)
% \AtlasCoverReaderMember{Reader~1, Reader~2}
% \AtlasCoverReaderMember{Reader~1}
% \AtlasCoverEdBoardMember{Reader~2}

% Editors egroup
\AtlasCoverEgroupEditors{atlas-STDM-2014-04-editors@cern.ch}

% EdBoard egroup
\AtlasCoverEgroupEdBoard{atlas-STDM-2014-04-editorial-board@cern.ch}

